GeoTopoDiff: Learning Geometry--Topology Graph Priors through Boundary-Constrained Mixed Diffusion for Sparse-Slice 3D Porous Reconstruction

Diffusion-based voxel prior modelling is challenging for the reconstruction of large-scale 3D porous microstructures. Due to the demanding requirements for simultaneously modelling both the continuous pore morphology and the discrete pore-throat topology, the diffusion models require fully observed CT scans to provide topology-faithful priors, which results in an inherent trade-off among throughput, topological fidelity, and field of view in practical industrial applications. We propose GeoTopoDiff, a graph diffusion-based framework for reconstructing 3D porous microstructures from sparse CT slices. GeoTopoDiff transfers the learning of diffusion priors from a voxel-based space to a mixed graph state space, which simultaneously encompasses continuous pore geometry and discrete pore-throat topology. A topology-aware partial graph prior from sparsely observed CT slices is introduced to constrain the reverse denoising process. Experiments on anisotropic PTFE and Fontainebleau sandstone show that GeoTopoDiff reduces morphology-related errors by 19.8% and topology-sensitive transport errors by 36.5% on average. Our findings suggest that the mixed graph state space promotes the diffusion denoising process to reduce posterior uncertainty under a sparse observations. All models and code have been made publicly available to facilitate the exploration of diffusion models in the field of 3D porous microstructures simulation.

==> Neurips/checklist.tex <==

\section*{NeurIPS Paper Checklist}

\begin{enumerate}[leftmargin=1.5em]
\item \textbf{Claims.} \answerYes{} The main claims are stated in the abstract and Introduction, and are supported by the experiments in Section~\ref{sec:experiments}.
\item \textbf{Limitations.} \answerYes{} Limitations are discussed in Section~\ref{sec:conclusion}.
\item \textbf{Theory assumptions and proofs.} \answerNA{} The paper proposes an empirical reconstruction method and does not present formal theorems.
\item \textbf{Experimental reproducibility.} \answerYes{} The datasets, observation protocol, baselines, metrics, training objective, and sampling procedure are described in the main text and appendix. Hardware-specific profiling details should be filled in before final submission if required.
\item \textbf{Open access to data and code.} \answerNo{} This draft does not include a public code release. The PTFE data are in-house micro-CT scans and may be subject to release restrictions.
\item \textbf{Experimental setting and details.} \answerYes{} Section~\ref{sec:experiments} and Appendix~\ref{app:additional_results} describe the evaluation setting, metrics, and ablations.
\item \textbf{Statistical significance.} \answerYes{} The paper reports mean and variance over multiple stochastic reconstructions; additional tests can be added if required by the final experimental protocol.
\item \textbf{Compute resources.} \answerYes{} Relative efficiency statistics are reported in Appendix~\ref{tab:efficiency_app}. Exact hardware details should be added before submission.
\item \textbf{Code of ethics.} \answerYes{} The work concerns digital reconstruction of materials microstructures and does not involve human subjects or personally identifiable data.
\item \textbf{Broader impacts.} \answerYes{} Potential impact is discussed through applications to pore-scale modeling and transport-relevant materials analysis.
\item \textbf{Safeguards.} \answerNA{} No release of models that interact with users or safety-critical decisions is proposed in this draft.
\item \textbf{Licenses for existing assets.} \answerYes{} Public templates and cited datasets/methods should be used under their corresponding licenses; the project includes a legacy-template README.
\item \textbf{New assets.} \answerNA{} The draft does not release a new public dataset in its present form.
\item \textbf{Crowdsourcing and research with human subjects.} \answerNA{} No crowdsourcing or human-subject research is involved.
\end{enumerate}


==> Neurips/sections/00_abstract.tex <==

\begin{abstract}
Reconstructing a three-dimensional porous microstructure from two sparse micro-CT boundary slices is severely underdetermined: many visually plausible interiors can satisfy the same observations while exhibiting incompatible pore connectivity and transport behavior. We propose \method, a boundary-constrained mixed graph diffusion model for sparse-slice porous media reconstruction. Instead of generating the volume only in voxel space, \method{} represents the unknown interior as coupled continuous pore geometry and discrete pore-throat topology. A boundary graph extractor converts the observed top and bottom slices into a partial pore network, which conditions a mixed diffusion process through geometry--topology interaction blocks and boundary cross-attention. During sampling, observed boundary variables are clamped at every reverse step, yielding stochastic interiors that remain exactly consistent with the measured slices. On isotropic Fontainebleau sandstone and anisotropic fibrous PTFE, \method{} improves morphology descriptors, connected-cluster statistics, and transport-oriented evaluations over GAN-based and statistics-informed baselines. The results support the view that sparse slices constrain not only appearance but also a latent boundary network, and that making this network explicit improves topology-aware 3D reconstruction.
\end{abstract}


==> Neurips/sections/01_introduction.tex <==

\section{Introduction}

Three-dimensional characterization of porous media is central to pore-scale simulation and to the estimation of transport-relevant properties such as porosity, pore-size distribution, connectivity, and permeability \citep{Blunt2013PoreScale,Wildenschild2013Xray,Torquato2002RHM}. X-ray micro-computed tomography (micro-CT) can directly image such structures, but practical acquisition is constrained by a trade-off between field of view, spatial resolution, scan time, and dose. Dense scans preserve fine morphology and pore continuity, whereas sparse scans are cheaper and cover larger domains but leave large interior regions unobserved. Reconstructing the missing interior from only a few slices is therefore not a deterministic interpolation problem; it is a conditional sampling problem over plausible microstructures.

This ambiguity is especially consequential for porous media. A reconstruction can match local texture or low-order correlation statistics while breaking percolating pathways that dominate permeability. Classical descriptor-matching methods and multiple-point statistics provide interpretable constraints, but they are often computationally expensive and can struggle with long-range connectivity in heterogeneous samples \citep{Yeong1998RandomMediaII,Bostanabad2018Review}. Deep generative models, including GAN-based 2D-to-3D reconstruction and recent diffusion models, have improved realism and sampling speed \citep{Mosser2017PRE,Mosser2018TPM,Kench2021SliceGAN,Feng2020EndToEnd,Fu2023SINN,Ho2020DDPM,Lee2024Micro3Diff}. However, most of these approaches operate primarily in voxel space. Connectivity, pore adjacency, and throat structure are learned only implicitly, so topology can remain fragile under sparse boundary conditioning.

Our key observation is that sparse boundary slices provide more than image appearance: they reveal a partial pore network on the observed boundaries. Treating this partial network as an explicit condition narrows the posterior over plausible interiors. We therefore formulate sparse-slice reconstruction as \emph{boundary-conditioned porous graph completion}. Boundary pores define observed nodes with measured geometry, while the unknown interior is represented by continuous geometric variables and discrete topological variables. This formulation separates what is naturally continuous, such as pore centroids and radii, from what is naturally combinatorial, such as node states and pore-throat connectivity.

We instantiate this idea in \method, a topology-aware mixed graph diffusion framework. A boundary graph extractor segments the observed slices, lifts pore instances to boundary nodes, and constructs a partial graph prior. Conditioned on this prior, \method{} jointly denoises continuous geometry and discrete topology with a mixed diffusion process. Geometry--topology interaction blocks allow candidate throats to influence pore updates and pore geometry to influence throat updates, while boundary cross-attention anchors the denoising trajectory to the observed graph. At inference time, freeze-and-update sampling clamps boundary variables after every reverse step, enforcing exact boundary consistency while retaining posterior diversity in the unobserved interior.

Our contributions are as follows.
\begin{itemize}
    \item We cast sparse-slice porous media reconstruction as boundary-conditioned posterior sampling over coupled geometry and topology, rather than as voxel-only interpolation.
    \item We introduce \method, a mixed graph diffusion model that jointly denoises continuous pore geometry and discrete pore-throat topology under a partial boundary graph prior.
    \item We evaluate on isotropic sandstone and anisotropic fibrous PTFE, showing improved morphology, topology, and transport-oriented consistency over representative GAN-based and statistics-informed baselines.
\end{itemize}


==> Neurips/sections/02_related_work.tex <==

\section{Related work}

\paragraph{Porous media reconstruction from limited observations.}
Early reconstruction methods generated random media by matching statistical descriptors, simulated annealing objectives, Gaussian fields, or multiple-point statistics \citep{Yeong1998RandomMediaII,Bostanabad2018Review,Torquato2002RHM}. These methods remain attractive because their constraints are physically interpretable, but their iterative nature can be costly and long-range connectivity is difficult to preserve when the observations are sparse. Deep generative models shifted reconstruction toward amortized sampling. GAN-based methods have been used for 3D porous media synthesis \citep{Mosser2017PRE,Mosser2018TPM} and dimensionality expansion from 2D slices \citep{Kench2021SliceGAN,Valsecchi2020GAN,Feng2020EndToEnd,Zhang2021SliceToVoxel,Volkhonskiy2022GAN}. Statistics-informed neural approaches further incorporate descriptor losses to improve structural consistency \citep{Fu2023SINN}. Our work is complementary: it targets sparse boundary-conditioned reconstruction and adds an explicit graph prior for topology.

\paragraph{Topology-aware representations.}
Pore-network modeling abstracts a porous medium as pores connected by throats, providing a compact representation for flow and transport analysis \citep{Blunt2013PoreScale,Xiong2016PoreNetworkReview}. Recent graph neural networks use related representations for property prediction and digital rock analysis, illustrating that graph connectivity carries information not easily captured by local voxel descriptors. Most such work uses graphs as downstream analysis tools. In contrast, \method{} uses a partial pore graph as a generative condition and reconstructs the hidden interior topology during sampling.

\paragraph{Diffusion models for structured generation.}
Denoising diffusion probabilistic models provide stable likelihood-based training and broad mode coverage for continuous data \citep{Ho2020DDPM}. Discrete diffusion extends the same denoising principle to categorical state spaces through Markov corruption processes \citep{Austin2021D3PM}. In materials and microstructure generation, diffusion has recently been used for descriptor-consistent reconstruction and 2D-to-3D dimensionality expansion \citep{Lee2024Micro3Diff,Dureth2023Diffusion}. \method{} differs by modeling two variable types simultaneously: continuous geometry and discrete topology. This mixed formulation is designed for porous graph completion, where the topology of the generated structure is as important as its visual appearance.


==> Neurips/sections/03_method.tex <==

\section{GeoTopoDiff}
\label{sec:method}

\subsection{Boundary-conditioned graph completion}

Let $X\in\{0,1\}^{H\times W\times D}$ denote a binary porous volume, where one phase represents pore space. The observation is a pair of boundary slices $Y=\{I^{\mathrm{bot}}, I^{\mathrm{top}}\}$ with $I^{\mathrm{bot}}=X[:,:,1]$ and $I^{\mathrm{top}}=X[:,:,D]$. The goal is to sample plausible interiors $X[:,:,2:D-1]$ conditioned on $Y$.

We represent a porous microstructure by a graph state
\begin{equation}
\mathcal S_t=(\mathbf B_t,\mathbf C_t,\mathbf E_t),
\end{equation}
where $t$ is the diffusion step. For pore node $i$, $b_{i,t}=[x_{i,t},y_{i,t},z_{i,t},r_{i,t}]\in\R^4$ denotes centroid and equivalent radius, $c_{i,t}\in\{1,\ldots,K_c\}$ denotes a node label, and $e_{ij,t}\in\{0,\ldots,K_e-1\}$ denotes the label of candidate edge $(i,j)\in\mathcal I$. In the binary setting, $e_{ij,t}=1$ indicates a pore-throat connection and $e_{ij,t}=0$ indicates no connection.

A boundary graph extractor maps $Y$ to a partial graph prior $\tilde{\mathcal S}=(\tilde{\mathbf B},\tilde{\mathbf C},\tilde{\mathbf E})$. Each boundary slice is segmented with a U-Net-style mask predictor \citep{Ronneberger2015UNet}; connected pore components yield 2D centroids and equivalent radii; bottom and top components are lifted to $z=0$ and $z=D$, respectively. Reliable local boundary relations are added as observed edges. The resulting graph is partial by construction: it fixes boundary evidence but leaves the interior geometry and hidden throats unresolved. We learn the conditional posterior
\begin{equation}
    p_\theta(\mathcal S_0\mid \tilde{\mathcal S},Y),
\end{equation}
where $\mathcal S_0$ is the clean porous graph.

\begin{figure}[H]
    \centering
    \todofig{1_overview.pdf}{0.95\linewidth}
    \caption{Overview of \method. Observed top and bottom micro-CT slices are converted into a partial boundary graph. A mixed graph diffusion model then reconstructs continuous pore geometry and discrete pore-throat topology while clamping observed boundary variables during reverse sampling.}
    \label{fig:overview}
\end{figure}

\subsection{Mixed diffusion over geometry and topology}

\paragraph{Continuous geometry.}
Geometry variables are corrupted with Gaussian noise as in DDPMs:
\begin{equation}
q_c(\mathbf B_t\mid\mathbf B_0)=\prod_{i=1}^N
\mathcal N\left(b_{i,t};\sqrt{\bar\alpha_t}\,b_{i,0},(1-\bar\alpha_t)\mathbf I\right),
\label{eq:cont_forward}
\end{equation}
where $\bar\alpha_t=\prod_{s=1}^t\alpha_s$. Equivalently,
\begin{equation}
 b_{i,t}=\sqrt{\bar\alpha_t}\,b_{i,0}+\sqrt{1-\bar\alpha_t}\,\epsilon_i,
 \quad \epsilon_i\sim\mathcal N(0,\mathbf I).
\end{equation}

\paragraph{Discrete topology.}
Node and edge labels are corrupted with categorical Markov transitions following discrete diffusion:
\begin{align}
q_d(\mathbf C_t\mid\mathbf C_0)&=\prod_{i=1}^N \Cat(c_{i,t};c_{i,0}\bar{\mathbf Q}^{c}_t),\\
q_d(\mathbf E_t\mid\mathbf E_0)&=\prod_{(i,j)\in\mathcal I} \Cat(e_{ij,t};e_{ij,0}\bar{\mathbf Q}^{e}_t),
\end{align}
where $\bar{\mathbf Q}_t=\mathbf Q_1\cdots\mathbf Q_t$ and the transition matrices include a terminal corruption state. The mixed forward process factorizes over the continuous and discrete branches:
\begin{equation}
q(\mathcal S_t\mid\mathcal S_{t-1})=q_c(\mathbf B_t\mid\mathbf B_{t-1})q_d(\mathbf C_t\mid\mathbf C_{t-1})q_d(\mathbf E_t\mid\mathbf E_{t-1}).
\end{equation}

\paragraph{Reverse denoising.}
The reverse model predicts a geometry denoising signal and categorical posteriors for node and edge labels:
\begin{align}
&p_\theta(\mathcal S_{t-1}\mid\mathcal S_t,\tilde{\mathcal S},t) \\
&\quad =p_\theta^b(\mathbf B_{t-1}\mid\mathcal S_t,\tilde{\mathcal S},t)
 p_\theta^c(\mathbf C_{t-1}\mid\mathcal S_t,\tilde{\mathcal S},t)
 p_\theta^e(\mathbf E_{t-1}\mid\mathcal S_t,\tilde{\mathcal S},t).
\label{eq:reverse_factor}
\end{align}

\subsection{Boundary-aware denoising architecture}

At reverse step $t$, node and edge states are embedded as
\begin{align}
h_i^{(0)} &= \phi_b(b_{i,t})\oplus\phi_c(c_{i,t})\oplus\phi_t(t),\\
g_{ij}^{(0)} &= \phi_e(e_{ij,t})\oplus\phi_\delta(\delta_{ij,t})\oplus\phi_t(t),
\end{align}
where $\oplus$ denotes concatenation and
\begin{equation}
\delta_{ij,t}=\big[x_{i,t}-x_{j,t},y_{i,t}-y_{j,t},z_{i,t}-z_{j,t},r_{i,t}-r_{j,t},\|p_{i,t}-p_{j,t}\|_2\big].
\end{equation}
The boundary graph is encoded using the same geometry, label, and relative-position embeddings.

\begin{figure}[H]
    \centering
    \todosmallfig{2_GeoTopDiff.pdf}{0.95\linewidth}
    \caption{Denoising block. Node and edge features are updated jointly by geometry--topology interaction, modulated with time conditioning, and anchored to the observed boundary graph through cross-attention.}
    \label{fig:architecture}
\end{figure}

Each denoising block has three components. First, adaptive normalization injects the diffusion time. Second, a geometry--topology interaction module passes messages between nodes and candidate edges. Nodes aggregate geometry-aware neighbor information,
\begin{equation}
 m_i^h=\sum_{j\in\mathcal N(i)}\mathrm{softmax}_j\!\left(\frac{Q_i^h(K_{ij}^h)^\top}{\sqrt d}\right)V_{ij}^h,
\end{equation}
while each candidate edge aggregates information from its incident node pair,
\begin{equation}
 m_{ij}^e=\mathrm{softmax}\!\left(\frac{Q_{ij}^e(K_{ij}^e)^\top}{\sqrt d}\right)V_{ij}^e.
\end{equation}
The two branches are coupled with FiLM modulation \citep{Perez2018FiLM}. Node contexts modulate edge features, and incident edge contexts modulate node features:
\begin{align}
\tilde g_{ij}^{(l)} &= \gamma_{ij}^e\odot\mathrm{LN}(g_{ij}^{(l)}+m_{ij}^e)+\beta_{ij}^e,\\
\tilde h_i^{(l)} &= \gamma_i^h\odot\mathrm{LN}(h_i^{(l)}+m_i^h)+\beta_i^h.
\end{align}
Third, boundary cross-attention uses current graph features as queries and encoded boundary graph features as keys and values. This lets every denoising step condition on measured boundary structure rather than only on a global slice embedding.

\subsection{Training and boundary-constrained sampling}

Training minimizes the sum of continuous and discrete denoising losses:
\begin{equation}
\mathcal L=\lambda_b\mathcal L_{\mathrm{geo}}+\lambda_c\mathcal L_{\mathrm{node}}+\lambda_e\mathcal L_{\mathrm{edge}},
\end{equation}
with
\begin{align}
\mathcal L_{\mathrm{geo}}&=\mathbb E\sum_i\left\|\epsilon_i-\hat\epsilon_{i,\theta}(\mathcal S_t,\tilde{\mathcal S},t)\right\|_2^2,\\
\mathcal L_{\mathrm{node}}&=\mathbb E\sum_i \KL\!\left(q(c_{i,t-1}\mid c_{i,t},c_{i,0})\,\|\,p_\theta^c(c_{i,t-1}\mid\mathcal S_t,\tilde{\mathcal S},t)\right),\\
\mathcal L_{\mathrm{edge}}&=\mathbb E\sum_{(i,j)\in\mathcal I} \KL\!\left(q(e_{ij,t-1}\mid e_{ij,t},e_{ij,0})\,\|\,p_\theta^e(e_{ij,t-1}\mid\mathcal S_t,\tilde{\mathcal S},t)\right).
\end{align}

At inference time, observed boundary variables are treated as hard constraints. Interior variables are initialized from their terminal priors. After each reverse update, all boundary nodes and observed boundary-supported edges are overwritten by their values in $\tilde{\mathcal S}$. Algorithm~\ref{alg:sampling} summarizes this freeze-and-update sampler.

\begin{algorithm}[H]
\caption{Boundary-constrained reverse sampling}
\label{alg:sampling}
\begin{algorithmic}[1]
\STATE \textbf{Input:} boundary slices $Y$, trained model $p_\theta$, steps $T$
\STATE Extract partial boundary graph $\tilde{\mathcal S}$ from $Y$
\STATE Initialize unknown interior variables from terminal geometry and categorical priors
\STATE Set observed boundary variables to $\tilde{\mathcal S}$
\FOR{$t=T,T-1,\ldots,1$}
    \STATE Predict $\hat\epsilon_{\mathbf B}$, $p_\theta(\mathbf C_{t-1})$, and $p_\theta(\mathbf E_{t-1})$
    \STATE Update only unknown interior geometry and topology
    \STATE Clamp all observed boundary variables back to $\tilde{\mathcal S}$
\ENDFOR
\STATE \textbf{return} reconstructed porous graph $\hat{\mathcal S}_0$
\end{algorithmic}
\end{algorithm}


==> Neurips/sections/04_experiments.tex <==

\section{Experiments}
\label{sec:experiments}

We evaluate whether explicit topology modeling improves sparse-slice reconstruction under the same boundary observations. The main text reports the results most relevant to the central claims; extended curves, sensitivity analyses, and efficiency measurements are provided in Appendix~\ref{app:additional_results}.

\subsection{Experimental setup}

\paragraph{Datasets.}
We use two binary porous-media regimes. The first is Fontainebleau sandstone, a standard isotropic digital-rock benchmark for pore-scale reconstruction and permeability-sensitive evaluation. The second is an in-house fibrous PTFE micro-CT dataset acquired with a Zeiss Xradia Versa 620 system. The PTFE volume has strong directional heterogeneity caused by aligned fiber bundles, making it a challenging test for anisotropic reconstruction. All experiments use $128^3$ crops with top and bottom slices as observations.

\paragraph{Baselines.}
We compare against three representative baselines: SliceGAN \citep{Kench2021SliceGAN}, a GAN-based dimensionality-expansion method; SAGAN \citep{Zhang2019SAGAN}, a self-attention GAN baseline with stronger global modeling; and SINN \citep{Fu2023SINN}, a statistics-informed neural reconstruction method designed to preserve morphology and connectivity descriptors. All methods are trained or adapted to output $128^3$ volumes and receive the same boundary observations at test time.

\paragraph{Metrics.}
We evaluate morphology with two-point correlation functions (TPCF) and pore-size distributions (PSD), topology with connected-cluster distribution probability (CDP), and transport consistency with single-phase flow simulation and permeability relative error. For stochastic reconstructions, we report descriptor discrepancy and variance across multiple posterior samples under identical boundary constraints.

\subsection{Isotropic sandstone: topology matters beyond appearance}

Table~\ref{tab:sandstone_main} reports the main quantitative results on Fontainebleau sandstone. \method{} obtains the lowest morphology error, topology error, and posterior variance. The largest relative gain is in topology error, indicating that the boundary graph prior and mixed topology denoising address a failure mode that is not captured by visual realism alone.

\begin{table}[H]
\caption{Fontainebleau sandstone reconstruction. Errors are computed from descriptor discrepancies against reference micro-CT volumes; lower is better.}
\label{tab:sandstone_main}
\centering
\begin{tabular}{lccc}
\toprule
Method & Morphology error $\downarrow$ & Topology error $\downarrow$ & Diversity var. $\downarrow$ \\
\midrule
SliceGAN & $0.0030\pm0.0010$ & $0.0012\pm0.0004$ & $0.0017$ \\
SAGAN & $0.0014\pm0.0008$ & $0.0010\pm0.0004$ & $0.0018$ \\
SINN & $0.0080\pm0.0020$ & $0.0034\pm0.0008$ & $0.0023$ \\
\method{} & $\mathbf{0.0010\pm0.0005}$ & $\mathbf{0.0002\pm0.0001}$ & $\mathbf{0.0012}$ \\
\bottomrule
\end{tabular}
\end{table}

Figure~\ref{fig:tpcf_sandstone} shows the same trend through TPCF curves. \method{} tracks the reference curve most closely over short and long distances, while GAN baselines deviate more strongly at local scales and SINN shows larger descriptor spread. The improvement in CDP, reported in Appendix~\ref{app:additional_results}, suggests that the gain comes from preserving connected pore clusters rather than merely matching low-order statistics.

\begin{figure}[H]
    \centering
    \todosmallfig{3_TPCF.pdf}{0.95\linewidth}
    \caption{TPCF comparison on Fontainebleau sandstone. \method{} matches the reference descriptor more closely across distances, indicating improved morphology and long-range phase arrangement.}
    \label{fig:tpcf_sandstone}
\end{figure}

\paragraph{Transport consistency.}
Permeability is sensitive to small connectivity errors. Across posterior samples, \method{} gives lower permeability error and lower sample-to-sample variance than the baselines. This supports the central design choice: explicitly modeling pore-throat topology improves the functional quality of the reconstructed volume, not only its visual similarity.

\subsection{Anisotropic PTFE: preserving directional structure}

The PTFE case tests whether the method can reconstruct directional heterogeneity from only two boundary slices. Figure~\ref{fig:ptfe_qualitative} compares 3D reconstructions and orthogonal cross-sections. \method{} better preserves elongated void regions and aligned channel continuity, while the baselines exhibit stronger local fragmentation and cross-plane inconsistency.

\begin{figure}[H]
    \centering
    \todofig{7_3D_view.pdf}{0.95\linewidth}
    \caption{PTFE reconstruction and orthogonal slices. \method{} better preserves anisotropic void alignment and cross-plane continuity under the same sparse boundary observations.}
    \label{fig:ptfe_qualitative}
\end{figure}

Figure~\ref{fig:ptfe_tpcf} reports TPCF-based relative error, variance, and KL divergence for the YZ, XZ, and XY planes. \method{} is consistently better across planes, with the strongest improvement at medium and long distances, where directional continuity is most visible. Air-flow simulation results in Appendix~\ref{app:additional_results} show that this structural improvement translates to more faithful velocity-field organization.

\begin{figure}[H]
    \centering
    \todosmallfig{8_TPCF_case2.pdf}{0.95\linewidth}
    \caption{Directional TPCF evaluation on PTFE. \method{} achieves lower error, lower variance, and lower KL divergence across YZ, XZ, and XY planes.}
    \label{fig:ptfe_tpcf}
\end{figure}

\subsection{Ablation study}

Table~\ref{tab:ablation_main} isolates the role of each component on PTFE. Removing the boundary graph prior causes the largest degradation, confirming that explicit structural conditioning reduces sparse-slice ambiguity. Removing discrete topology diffusion also degrades results substantially, indicating that continuous pore geometry alone is insufficient for connectivity preservation. Geometry--topology interaction and boundary cross-attention provide additional gains by coupling node and edge reasoning and keeping denoising anchored to measured boundary evidence.

\begin{table}[H]
\caption{Component ablation on anisotropic PTFE. Values average the YZ, XZ, and XY plane metrics; lower is better.}
\label{tab:ablation_main}
\centering
\begin{tabular}{llccc}
\toprule
Variant & Removed component & RelErr $\downarrow$ & Var. $\downarrow$ & KL $\downarrow$ \\
\midrule
Full & -- & \textbf{0.0085} & \textbf{0.0011} & \textbf{0.0042} \\
M1 & boundary graph prior & 0.0164 & 0.0024 & 0.0099 \\
M2 & discrete topology diffusion & 0.0134 & 0.0020 & 0.0078 \\
M3 & geometry--topology interaction & 0.0113 & 0.0016 & 0.0063 \\
M4 & boundary cross-attention & 0.0102 & 0.0014 & 0.0055 \\
\bottomrule
\end{tabular}
\end{table}


==> Neurips/sections/05_conclusion.tex <==

\section{Discussion and conclusion}
\label{sec:conclusion}

We presented \method, a boundary-constrained mixed graph diffusion model for sparse-slice porous media reconstruction. The method makes topology explicit by representing the hidden interior through continuous pore geometry and discrete pore-throat variables. A partial boundary graph extracted from the observed slices conditions the reverse process, and freeze-and-update sampling enforces exact consistency with measured boundary variables. Experiments on isotropic sandstone and anisotropic PTFE show that this design improves morphology, topology, and transport-oriented evaluations over representative GAN-based and statistics-informed baselines.

The approach also has limitations. The boundary graph is only as reliable as the segmentation and graph lifting used to construct it, and the present formulation conditions on top--bottom boundary slices rather than arbitrary sparse observation patterns. Transport agreement is improved indirectly through topology-aware generation rather than through a differentiable physics objective. Future work should integrate graph and voxel generation more tightly, study multi-phase porous materials, and incorporate property-aware losses or differentiable flow solvers when target transport properties are available.


==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and introduction state the main contributions: mixed geometry--topology graph diffusion, partial boundary graph conditioning, and sparse-boundary \(\mu\)CT porous reconstruction. 

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Appendix \ref{app:limitations} outlines the limitations of the proposed method.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper does not present formal theoretical theorems. but some theoretical foundations for the algorithms used are provided in Appendix \ref{app:method_details}.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper describes the sparse-boundary evaluation protocol, datasets, train/validation/test splits, baseline adaptations, metrics, permeability simulation protocol, model components, and ablation settings. The method section and appendix specify the graph extraction, mixed diffusion process, boundary graph construction, decoder, loss terms, and sampling procedure.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}.
    \item[] Justification: We provide implementation code in the supplementary material. The de-anonymized public GitHub link, full code release, trained checkpoints, and complete data-access instructions will be included in the camera-ready version.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The experiments specify the two datasets, crop size, split sizes, sparse-boundary observation protocol, baseline conditioning mechanisms, evaluation metrics, permeability solver, and ablation variants. Model and diffusion details are described in the method section and appendix.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The main tables report metrics averaged over test samples and posterior samples, all main results include standard deviations. Full statistical significance tests are not included due to the computational cost of repeated 3D diffusion sampling and permeability simulation.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The compute resources and runtime for the experiments are specified in terms of normalized parameter count, peak GPU memory, training time, and sampling time for ablated variants. However, the current draft does not provide complete absolute hardware specifications and wall-clock costs for every baseline.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work studies reconstruction of porous material microstructures from \(\mu\)CT data and does not involve human subjects, personal data, surveillance, deception, or high-risk decision making. The authors have reviewed the NeurIPS Code of Ethics and are not aware of any deviation.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper discusses the potential positive impact of reducing the need for dense high-quality \(\mu\)CT scans in porous material characterization and high-throughput industrial imaging. It also notes limitations and possible risks if reconstructed volumes are used for transport prediction without validation, especially because transport agreement is improved indirectly rather than through a differentiable physics objective.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not release high-risk generative models, scraped datasets, personal data, or models that can generate human-facing harmful content. 

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}.
    \item[] Justification: Sandstone dataset used in this paper is from the public domain.  PTFE dataset from the private domain, information will be added when the code and data access package is finalized.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}.
    \item[] Justification:  We have cited all works and datasets that this paper uses.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing, human annotation, user studies, or research with human subjects.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve human subjects, personal data, clinical data, or crowdsourcing, so IRB approval or equivalent human-subjects review is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerNA{}.
    \item[] Justification: The core method does not use LLMs as an important, original, or non-standard component. Any use of language models for writing, editing, and formatting assistance does not affect the methodology, experiments, scientific rigor, and originality of the research.

\end{enumerate}
